Progenitor, Precursor and Evolution of the Dusty Remnant of the Stellar Merger M31-LRN-2015

M31-2015-LRN is a likely stellar merger discovered in the Andromeda Galaxy in 2015. We present new optical to mid-infrared photometry and optical spectroscopy for this event. Archival data shows that the source started to brighten $\sim$2 years before the nova event. During this precursor phase, the source brightened by $\sim$3 mag. The lightcurve at 6 and 1.5 months before the main outburst may show periodicity, with periods of 16$\pm$0.3 and 28.1$\pm$1.4 days respectively. This complex emission may be explained by runaway mass loss from the system after the binary undergoes Roche-lobe overflow, leading the system to coalesce in tens of orbital periods. While the progenitor spectral energy distribution shows no evidence of pre-existing warm dust in system, the remnant forms an optically thick dust shell at $\sim$4 months after the outburst peak. The optical depth of the shell increases dramatically after 1.5 years, suggesting the existence of shocks that enhance the dust formation process. We propose that the merger remnant is likely an inflated giant obscured by a cooling shell of gas with mass $\sim0.2$ M$_{\odot}$ ejected at the onset of the common envelope phase.

==> photometry_figure3.tex <==
\begin{table}
\begin{center}
\begin{minipage}{16cm}
\caption{Photometry}
\label{tab:photometry}
\begin{tabular}{llllll}
\hline
\hline
{Phase} & {MJD} & {Telescope} & {Filter} & {Magnitude} & {Refs.} \\ 
\hline
Phase     & MJD    & Telescope  & Filter & Magnitudes      & ATEl         \\
-3810.7 & 53233 & HST        & I      & 22.02$\pm$0.01  & 7173        \\
-3810.7 & 53233 & HST        & V      & 23.2$\pm$0.03   & 7173        \\
-3443.7 & 53600 & Spitzer      & 3.6      &       $>$17.99        &         \\
-3443.7 & 53600 & Spitzer      & 4.5      &       $>$17.83        &         \\
-3443.7 & 53600 & Spitzer      & 5.8      &       $>$17.03        &         \\
-3443.7 & 53600 & Spitzer      & 8.0      &       $>$15.89        &         \\
-1968.7 & 55075 & CFHT       & g      & 22.6$\pm$0.0    & 7173        \\
-89.7    & 56954 & CFHT       & g      & 20.8$\pm$0.0    & 7173        \\
-8.7     & 57035 & Kislovodsk & W      & 18.73$\pm$0.08  & 6951        \\
-8.7     & 57035 & Kislovodsk & unfilt & 19.0$\pm$0.0    & 6911        \\
-8.7     & 57035 & Kislovodsk & W      & 16.02$\pm$0.02  & 6951        \\
-8.7     & 57035 & Schmidt    & R      & 18.002$\pm$0.03 & 6924        \\
-8.7     & 57035 & Schmidt    & B      & 19.503$\pm$0.06 & 6924        \\
-7.7     & 57036 & Kislovodsk & W      & 17.79$\pm$0.08  & 6951        \\
-7.7     & 57036 & Schmidt    & R      & 16.82$\pm$0.019 & 6924        \\
-7.7     & 57036 & Schmidt    & Ha     & 16.81$\pm$0.028 & 6924        \\
-6.7     & 57037 & Kislovodsk & W      & 16.6$\pm$0.04   & 6951        \\
-6.7     & 57037 & BTA        & B      & 17.06$\pm$0.04  & 6985        \\
-6.7     & 57037 & BTA        & V      & 16.4$\pm$0.02   & 6985        \\
-6.7     & 57037 & BTA        & R      & 15.99$\pm$0.02  & 6985        \\
-6.7     & 57037 & Schmidt    & R      & 16.018$\pm$0.02 & 6941        \\
-6.7     & 57037 & Schmidt    & R      & 15.981$\pm$0.01 & 6941        \\
-6.7     & 57037 & Schmidt    & B      & 16.965$\pm$0.03 & 6941        \\
-5.7     & 57038 & Kislovodsk & W      & 16.02$\pm$0.01  & 6951        \\
-5.7     & 57038 & Schmidt    & B      & 16.521$\pm$0.02 & 6941        \\
-5.7     & 57038 & Schmidt    & R      & 15.633$\pm$0.02 & 6941        \\
-5.7     & 57038 & Schmidt    & R      & 15.598$\pm$0.01 & 6941        \\
-4.7     & 57039 & Tunka      & W      & 15.87$\pm$0.02  & 6951        \\
-4.7     & 57039 & Tunka      & V      & 15.77$\pm$0.04  & 6951        \\
-4.7     & 57039 & Tunka      & W      & 15.89$\pm$0.04  & 6951        \\
-4.7     & 57039 & Tunka      & V      & 15.71$\pm$0.07  & 6951        \\
-4.7     & 57039 & Kislovodsk & W      & 15.81$\pm$0.02  & 6951        \\
-4.7     & 57039 & Kislovodsk & W      & 15.83$\pm$0.03  & 6951        \\
-4.7     & 57039 & Kislovodsk & W      & 15.69$\pm$0.01  & 6951        \\
-4.7     & 57039 & Kislovodsk & W      & 15.71$\pm$0.01  & 6951        \\
-4.7     & 57039 & Kislovodsk & R      & 15.42$\pm$0.01  & 6951        \\
-3.7     & 57040 & Tunka      & I      & 15.26$\pm$0.06  & 6951        \\
-3.7     & 57040 & Tunka      & W      & 15.56$\pm$0.01  & 6951        \\
-3.7     & 57040 & Tunka      & I      & 15.08$\pm$0.06  & 6951        \\
-3.7     & 57040 & Tunka      & W      & 15.54$\pm$0.01  & 6951        \\
-3.7     & 57040 & Tunka      & I      & 15.1$\pm$0.05   & 6951        \\
-3.7     & 57040 & Tunka      & W      & 15.51$\pm$0.01  & 6951        \\
-3.7     & 57040 & Tunka      & R      & 15.37$\pm$0.02  & 6951        \\
-3.7     & 57040 & Tunka      & R      & 15.45$\pm$0.02  & 6951        \\
-3.7     & 57040 & Kislovodsk & W      & 15.57$\pm$0.02  & 6951        \\
-3.7     & 57040 & Kislovodsk & W      & 15.62$\pm$0.02  & 6951        \\
-3.7     & 57040 & Kislovodsk & W      & 15.56$\pm$0.02  & 6951        \\
-3.7     & 57040 & Kislovodsk & R      & 15.39$\pm$0.02  & 6951        \\
-3.7     & 57040 & Kislovodsk & W      & 15.57$\pm$0.01  & 6951        \\
-3.7     & 57040 & Kislovodsk & R      & 15.39$\pm$0.02  & 6951        \\
-0.7     & 57043 & BTA        & B      & 15.94$\pm$0.03  & 6985        \\
-0.7     & 57043 & BTA        & V      & 15.41$\pm$0.01  & 6985        \\
-0.7     & 57043 & BTA        & R      & 15.09$\pm$0.01  & 6985        \\
2.3       & 57046 & McDonald   & B      & 16.0$\pm$0.04   & 7150        \\
2.3       & 57046 & McDonald   & R      & 15.24$\pm$0.02  & 7150        \\
16.3      & 57060 & Schmidt    & B      & 17.86$\pm$0.05  & 7150        \\
16.3      & 57060 & Schmidt    & R      & 15.74$\pm$0.03  & 7150        \\
27.3      & 57071 & Schmidt    & B      & 18.48$\pm$0.12  & 7150        \\
27.3      & 57071 & Schmidt    & I      & 15.22$\pm$0.03  & 7150        \\
27.3      & 57071 & Schmidt    & R      & 15.9$\pm$0.03   & 7150        \\
27.3      & 57071 & Schmidt    & V      & 16.87$\pm$0.04  & 7150        \\
30.3      & 57074 & BTA        & B      & 18.77$\pm$0.09  & 7150        \\
30.3      & 57074 & BTA        & R      & 15.84$\pm$0.03  & 7150        \\
30.3      & 57074 & BTA        & V      & 16.84$\pm$0.03  & 7150        \\
43.3      & 57087 & Mount Abu  & H      & 13.4$\pm$0.05   & 7236        \\
43.3      & 57087 & Mount Abu  & J      & 14.05$\pm$0.05  & 7236        \\
43.3      & 57087 & Mount Abu  & K      & 13.0$\pm$0.05   & 7236        \\
48.3      & 57092 & NOT        & B      & 20.06$\pm$0.05  & 7272        \\
48.3      & 57092 & NOT        & R      & 17.01$\pm$0.01  & 7272        \\
48.3      & 57092 & NOT        & I      & 15.56$\pm$0.02  & 7272        \\
51.3      & 57095 & NOT        & B      & 20.38$\pm$0.05  & 7272        \\
51.3      & 57095 & NOT        & R      & 17.32$\pm$0.01  & 7272        \\
51.3      & 57095 & NOT        & I      & 15.74$\pm$0.02  & 7272        \\
74.3      & 57118 & Spitzer    & 3.6    & 12.79$\pm$0.07  & 7468        \\
74.3      & 57118 & Spitzer    & 4.5    & 12.8$\pm$0.09   & 7468        \\
81.3      & 57125 & Spitzer    & 3.6    & 12.82$\pm$0.07  & 7468        \\
81.3      & 57125 & Spitzer    & 4.5    & 12.91$\pm$0.09  & 7468        \\
86.3      & 57130 & Spitzer    & 3.6    & 12.89$\pm$0.07  & 7485        \\
86.3      & 57130 & Spitzer    & 4.5    & 13.01$\pm$0.1   & 7485        \\
91.3      & 57135 & Spitzer    & 3.6    & 12.99$\pm$0.08  & 7485        \\
91.3      & 57135 & Spitzer    & 4.5    & 13.15$\pm$0.1   & 7485        \\
99.3      & 57143 & NOT        & I      & 21.1$\pm$0.3    & 7572        \\
99.3      & 57143 & NOT        & R      & $>$21.0       & 7572        \\
108.3     & 57152 & NOT        & I      & 21.6$\pm$0.2    & 7572        \\
113.3     & 57157 & SDSS       & i      & $>$21.0       & 7537        \\
121.3     & 57165 & Liverpool  & H      & 16.0$\pm$0.2    & 7555        \\
127.3     & 57171 & NOT        & H      & 16.1$\pm$0.1    & 7595        \\
127.3     & 57171 & NOT        & J      & 17.4$\pm$0.1    & 7595        \\
127.3     & 57171 & NOT        & K      & 14.7$\pm$0.1    & 7595        \\
128.3     & 57172 & NOT        & K      & 14.75$\pm$0.06  & 7624        \\
130.3     & 57174 & NOT        & H      & 16.31$\pm$0.07  & 7624        \\
130.3     & 57174 & NOT        & J      & 17.79$\pm$0.09  & 7624        \\
130.3     & 57174 & NOT        & K      & 14.74$\pm$0.06  & 7624        \\
131.3     & 57175 & NOT        & H      & 15.6$\pm$0.04   & 7624        \\
131.3     & 57175 & NOT        & J      & 17.34$\pm$0.12  & 7624        \\
131.3     & 57175 & NOT        & K      & 14.03$\pm$0.07  & 7624        \\
193.3     & 57237 & NOT        & J      & 18.362$\pm$0.1  & 8059        \\
193.3     & 57237 & NOT        & H      & 16.83$\pm$0.08  & 8059        \\
193.3     & 57237 & NOT        & K      & 15.05$\pm$0.06  & 8059        \\
224.3    & 57268 & NOT        & J      & 18.69$\pm$0.12  & 8059        \\
224.3    & 57268 & NOT        & H      & 16.94$\pm$0.07  & 8059        \\
224.3    & 57268 & NOT        & K      & 15.14$\pm$0.09  & 8059        \\
249.3    & 57293 & NOT        & J      & 18.89$\pm$0.12  & 8220        \\
249.3    & 57293 & NOT        & H      & 17.21$\pm$0.06  & 8220        \\
249.3    & 57293 & NOT        & K      & 15.34$\pm$0.08  & 8220        \\
264.3    & 57308 & Spitzer    & 3.6    & 13.72$\pm$0.11  &             \\
264.3    & 57308 & Spitzer    & 4.5    & 13.9$\pm$0.15   &             \\
271.3    & 57315 & Spitzer    & 3.6    & 13.74$\pm$0.11  &             \\
271.3    & 57315 & Spitzer    & 4.5    & 13.87$\pm$0.15  &             \\
278.3    & 57322 & Spitzer    & 3.6    & 13.72$\pm$0.11  &             \\
278.3    & 57322 & Spitzer    & 4.5    & 14.05$\pm$0.16  &             \\
435.3    & 57479 & Spitzer    & 3.6    & 14.85$\pm$0.19  &             \\
435.3    & 57479 & Spitzer    & 4.5    & 14.25$\pm$0.18  &             \\
571.3    & 57615 & Keck       & J      & 21.88$\pm$0.10  &             \\
571.3    & 57615 & Keck       & H      & 20.36$\pm$0.05  &             \\
571.3    & 57615 & Keck       & K      & 18.63$\pm$0.03  w&             \\
644.3    & 57688 & Spitzer    & 3.6    & 15.64$\pm$0.29  &             \\
644.3    & 57688 & Spitzer    & 4.5    & 14.26$\pm$0.18  &             \\
822.3    & 57866 & Spitzer    & 3.6    & 15.86$\pm$0.3   &             \\
822.3    & 57866 & Spitzer    & 4.5    & 14.36$\pm$0.2   &            \\
835.3     & 57879 & Spitzer    & 3.6    & 16.00$\pm$0.30 &              \\
835.3     & 57879 & Spitzer    & 4.5    & 14.42$\pm$0.30 &              \\
924.8     & 57968.5 & Keck       & J      & $>$24.4  &                  \\
924.8     & 57968.5 & Keck       & K      & 21.83$\pm$0.193   &         \\
1260.8    & 58304.5 & Keck       & K      & $>$24.26  &                 \\
1291.8    & 58335.5 & Keck       & J      & $>$25.27  &                 \\
1291.8    & 58335.5 & Keck       & H      & $>$24.81   &                \\
1793.2    & 58836.9 &  Spitzer  & 3.6   &  $>$17.2 & \\
1793.2    & 58836.9 &  Spitzer  & 4.5 & 15.73$\pm$0.02 & \\
\hline
\hline
\end{tabular}
\end{minipage}
\end{center}
\end{table}
